Stability Constrained Reinforcement Learning for Real-Time Voltage Control

Deep reinforcement learning (RL) has been recognized as a promising tool to address the challenges in real-time control of power systems. However, its deployment in real-world power systems has been hindered by a lack of formal stability and safety guarantees. In this paper, we propose a stability constrained reinforcement learning method for real-time voltage control in distribution grids and we prove that the proposed approach provides a formal voltage stability guarantee. The key idea underlying our approach is an explicitly constructed Lyapunov function that certifies stability. We demonstrate the effectiveness of the approach in case studies, where the proposed method can reduce the transient control cost by more than 30\% and shorten the response time by a third compared to a widely used linear policy, while always achieving voltage stability. In contrast, standard RL methods often fail to achieve voltage stability.

==> Preliminary.tex <==


% as summarized in the following proposition, though it leaves open the task of constructing such a Lyapunov function.
% \begin{proposition}[Lyapunov functions for stability~\cite{khalil2002nonlinear}]
% Consider a control system in~\eqref{eq:dyn} with equilibrium point $x_e$, i.e., $f(x_e, g_\theta(x_e)) = 0$. Suppose there exists a continuously differentiable function $V: \mathbb{R}^n \rightarrow \mathbb{R}$ such that
% \begin{align}
%     V(x_e) &= 0 \text{ and } V(x) > 0,\forall x\in \mathcal{D}-\{x_e\}\\
%     \dot{V}(x) &< 0,\forall x\in \mathcal{D}-\{x_e\}
% \end{align}
% Then the system is asymptotically stable at the equilibrium point $x_e$ and $V$ is called a Lyapunov function. If $V$ is further radially unbounded, i.e. $V(x)\rightarrow\infty$ as $\Vert x\Vert\rightarrow\infty$, then the system is globally asymptotically stable around $x_e$. 
%\end{proposition}

%This calls to the question on how to formally ensure stability during policy learning, and how to guarantee the learned policy is guaranteed to be stable. This will be the focus of the next section. 

==> Safe RL for Voltage Control (ACC)/Experiment.tex <==
% \todo{
% \begin{enumerate}
%     \item Voltage control: add a RL with regular NN baseline
%     \item Add a counter example: regular NN unstable v.s. Lya-RL stable
%     \item Add pendulum experiment
% \end{enumerate}}
% Note: the pendulum system represents a general class of robotic systems,
% $$M(q) \ddot{q} + C(q, \dot{q}) \dot{q} + g(q) = u(t)\,,$$

We end the paper with a case study demonstrating the effectiveness of our approach for stability constrained policy learning for voltage control. %{\color{blue}As our implementation uses DDPG, we name our approach as Stable-DDPG. } \guannan{We should say stable-ddpg is our approach somewhere. Does this make sense?} 

\textbf{Experimental Setup} Our evaluations focus on a Southern California Edison 56 bus distribution system with high penetration of photovoltaic (PV) generations. The detailed system parameters are given in~\cite{farivar2012optimal}. 
Figure \ref{fig:SCE56_bus} provides the 56-bus distribution circuit, where there are 5 PV generators and controllers located at Buses 18, 21, 30, 45 and 53. Simulations of the power system dynamics use pandapower~\cite{pandapower}.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{SCE56_bus.png}
    \caption{Schematic diagram of SCE 56 bus distribution system with PV generations.}
    \label{fig:SCE56_bus}
\end{figure}

% In addition, there are controllers at each PV bus, consisting of PV inverters and additional reactive devices that can supply and consume reactive power for voltage control. 
The nominal voltage magnitude at each bus is $12$kV, and the acceptable range for operation is $\pm 5\%$ of the nominal value which is $[11.4\text{kV}, 12.6\text{kV}]$. We simulate three different scenarios: 1) High voltages: the PV generators are generating large amount of power, this corresponds to the day-time scenario in California where there is abundant sunshine that can result in high voltage issues at some buses. 2) Low voltages: the system is serving heavy loads without PV generation. It corresponds to a nighttime scenario when there is no sunshine but significant load, which results in low voltage issues at some buses. 3) A mix of high and low voltages: there are both high PV generation and heavy loads, which results in a mixture of high voltage issues at some buses and low voltages at others. For each scenario, we vary the PV output and the load to obtain different voltage conditions. 

\textbf{Our Approach and Baselines}  We incorporate the monotone policy network design with DDPG~\cite{lillicrap2015continuous} to obtain the provable stable RL controller, and name our approach as Stable-DDPG. For baseline algorithms, we consider the following linear policy with deadband $d_i(v_i) = -[v_i - \overline{v}_i]^{+} + [\underline{v}_i - v_i]^{+}$ (where $[x]^+= \max(x,0)$), which has been proposed and widely used in the power system control community~\cite{li2014real,zhang2013local}. It guarantees stability but may lead to suboptimal control cost. We also compare the performance of Stable-DDPG against DDPG, which is suggested for voltage control in~\cite{wang_data-driven_2020}. Standard DDPG minimizes the control cost without a formal stability guarantee. Details about the implementation and hyperparameters of Stable-DDPG and DDPG are provided in Appendix-\ref{sec:simulation_detail}. %We use Pytorch to build all the RL models and run the training process in Google Colab with GPU acceleration.\guannan{The last sentence could go to appendix?}
%However, since conventional NN policies are generally not monotone from input to output thus does not satisfy the stability condition, there is no guarantee for global stability. 

\textbf{Experimental Results} Figure~\ref{fig:control_policy} illustrates the control policy that is learned from Stable-DDPG and the baseline linear control~\cite{li2014real}.
\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.48\textwidth]{policy.png}
    \caption{Visualization of DDPG, Stable-DDPG and linear control policy at 5 PV buses. The x-axis is voltage (unit: kV) and the y-axis is control action (unit: MVar).}
    \label{fig:control_policy}
\end{figure}
Standard DDPG does not guarantee stability and thus can lead to ``infinite’’ voltage recovery time and control cost. To obtain a reasonable comparison, we limit the max episode length to be $T= 100$, and compare the voltage recovery time (steps) and reactive power consumption (MVar) on 500 different voltage violation scenarios. Table~\ref{table:voltage_control} shows the results. In terms of control performance, the average voltage recovery time of Stable-DDPG is 31.96 steps, which saves about a third of the response time compared to the linear policy (48.38 steps). 
As the Stable-DDPG is able to drive back the voltage into normal operation state faster, the average transient control cost (computed as the sum of control cost before voltage stabilization) of Stable-DDPG is reduced by $33.38\%$ compared to the linear policy. The standard deviation is high since the recovery time and control effort under different voltage violation conditions can be quite different. 
In addition, the lack of stability guarantee of standard DDPG can lead to higher control and state violation cost, which reflects in Table~\ref{table:voltage_control} that the control performance of standard DDPG is worse than the stable DDPG when averaging all scenarios. 

%\adam{make sure numbers match what is quoted in the intro} 
%Figure~\ref{fig:voltage_control} shows the voltage control performance in three representative test scenarios under high/low/mixture voltage violation conditions. 
% \begin{table}[t]
% \centering
% \caption{Performance of linear and Stable-DDPG policies on 500 different voltage violation scenarios.}
%  \label{table:voltage_control}
%  \begin{tabular}{lcccc}
%     \toprule
%     & \multicolumn{2}{c}{Voltage recovery time (steps)}  & \multicolumn{2}{c}{Reactive power consumption $(\text{MVar})$}  \\
%     \cmidrule(r){2-5}
%     Method     & Mean     & Std & Mean & Std \\
%     \midrule
%     Linear & 48.38 & 19.57 & 179.08 &   129.03\\
%     Stable-DDPG & \textbf{31.96} & 14.49 & \textbf{119.30} & 89.05  \\
%     \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\caption{Performance of linear, DDPG and Stable-DDPG policies on 500 voltage violation scenarios. Note: reactive power consumption denotes the control cost.}
 \label{table:voltage_control}
 \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{2}{c}{Voltage recovery time (steps)}  & \multicolumn{2}{c}{Reactive power $(\text{MVar})$}  \\
    \cmidrule(r){2-5}
    Method     & Mean     & Std & Mean & Std \\
    \midrule
    Linear & 48.38 & 19.57 & 179.08 &   129.03\\
    Stable-DDPG & \textbf{31.96} & 14.49 & \textbf{119.30} & 89.05  \\
    DDPG & 42.87   & 38.32 &  152.53 & 175.62   \\
    \bottomrule
\end{tabular}
\end{table}

% \begin{table}[h]
% \centering
% \caption{Performance of linear and Stable-DDPG policies on the voltage violation scenarios where DDPG can stablize voltage. Note: reactive power consumption denotes the control cost.}
%  \label{table:voltage_control}
%  \begin{tabular}{lcccc}
%     \toprule
%     & \multicolumn{2}{c}{Voltage recovery time (steps)}  & \multicolumn{2}{c}{Reactive power consumption $(\text{MVar})$}  \\
%     \cmidrule(r){2-5}
%     Method     & Mean     & Std & Mean & Std \\
%     \midrule
%     Linear &  41.11   & 18.93 &  128.81 &   102.97\\
%     Stable-DDPG & 25.80 & 14.40 & 80.75 &  67.98  \\
%     DDPG & \textbf{18.38}    &  9.96 &  \textbf{41.09} & 39.86    \\
%     \bottomrule
% \end{tabular}
% \end{table}


% \begin{figure}[tbp]
% \centering
%     \begin{minipage}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/high_voltage2.png}
%         %\caption{High voltage}
%         \label{fig:high_voltage_example}
%     \end{minipage}
%     \begin{minipage}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/low_voltage2.png}
%         %\caption{Low voltage}
%         \label{fig:low_voltage_example}
%     \end{minipage}
%     \begin{minipage}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/mixture2.png}
%         %\caption{Mixture}
%         \label{fig:mixture_example}
%     \end{minipage}
% \caption{Comparison of the baseline linear controller~\cite{li2014real} and Stable-DDPG under high voltage (left), low voltage (middle) and mix of high and low voltages (right) scenarios.}
% \label{fig:voltage_control}
% \end{figure}

\begin{figure}[tbp]
\centering
\begin{minipage}[t]{0.15\textwidth}
  \centering\raisebox{\dimexpr \topskip-\height}{%
  \includegraphics[width=\textwidth]{high_voltageviolation2.png}}
  %\captionof{figure}{Voltage instability.}
  \label{fig:instability}
\end{minipage}
\begin{minipage}[t]{0.15\textwidth}
  \centering\raisebox{\dimexpr \topskip-\height}{%
  \includegraphics[width=\textwidth]{low_voltageviolation2.png}}
  %\captionof{figure}{Voltage instability.}
  \label{fig:instability}
\end{minipage}
\begin{minipage}[t]{0.15\textwidth}
  \centering\raisebox{\dimexpr \topskip-\height}{%
  \includegraphics[width=\textwidth]{DDPG_vs_Lya.png}}
  %\captionof{figure}{Voltage instability.}
  \label{fig:instability}
\end{minipage}
\caption{Voltage stability of DDPG and Stable-DDPG.}
\label{fig:voltage_violation}
\end{figure}

\begin{figure}[t!]
\centering
    \begin{minipage}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{solar_load.png}
        %\caption{PV and load profile}
        %\label{fig:solar_load}
    \end{minipage}
    \begin{minipage}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{voltage_wo_control.png}
        %\caption{Without control}
        %\label{fig:low_voltage_example}
    \end{minipage}
    \begin{minipage}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{voltage_w_RL_control.png}
        %\caption{With Stable-DDPG}
        %\label{fig:real_world}
    \end{minipage}
\caption{Stable-DDPG test with real-world load and PV generation dataset. Left plot is the PV and aggregated load. Right two plots are the voltage without control and with Stable-DDPG.}
\label{fig:real_world}
\end{figure}
Figure \ref{fig:voltage_violation} compares the ability to achieve voltage stability of DDPG and Stable-DDPG under various test scenarios. The left plot shows the histogram of over-voltage ratio (i.e., $(v_T-v_0)^{+}/{v_0}$) and the middle plot shows the under-voltage ratio (i.e., $(v_0-v_T)^{+}/{v_0}$). Our method achieves voltage stability in all scenarios, whereas DDPG may lead to voltage instability, with the final voltage beyond the $\pm 5\%$ range for 30-40\% test scenarios. 
This is a serious issue since large voltage deviations violate regulatory requirements \cite{regulator} and can cause cascading failures \cite{haes2019survey}. 
Figure~\ref{fig:voltage_violation} right shows a test case where DDPG leads to voltage instability at bus 21. 
%Such a voltage instability result in ``infinite'' voltage recovery time. Thus, we set a maximum simulation horizon $T = 100$ when comparing the performance of Stable-DDPG, DDPG and linear policy in Table~\ref{table:voltage_control}. 
%The reason for instability is that the RL approach is trained on finite number of episodes, and may not generalize well in unseen voltage violation scenarios. In contrast, the proposed stability aware approach provides natural generalizability and stability guarantee to all trajectories whether seen or unseen during training. 
%These comparisons highlight that for real-world power application, explicitly enforcing stability is necessary in order to maintain the system reliability and safety under all conditions. 

Finally, we test the proposed method using real-world data from DOE~\cite{qu2019optimal}. We simulate a massive solar penetration scenario where all buses are associated with PV and voltage controllers. 
%The PV generation is nonzero from 8AM to 7PM, peaks at noon, and has large fluctuations throughout the day. 
%We trained a single stable-DDPG policy and used it across all the bus without further hyper-parameter tuning.
We compare the voltage dynamics without voltage control and when Stable-DDPG is used. Corresponding to the time resolution of the PV and load trajectory, the proposed method adjust its control output every 6s. The voltage control results are given in Figure~\ref{fig:real_world}. There are severe voltage violations without control, due to the high volatility in load and PV generation. In contrast, Stable-DDPG quickly brings the voltage into the stable operation range, which further demonstrates its applicability in power system voltage control.

% \todo{To TSG}

% \todo{centralize training - student/teacher framework}

% \todo{Look for a larger network}

% \todo{more test cases}

% \todo{ablation study: measurement noise, delay}

==> Safe RL for Voltage Control (ACC)/Introduction.tex <==

To achieve high penetration of distributed renewable generations at the distribution grid level, maintaining the voltage levels within the safe limit has been increasingly challenging.  Recently, significant efforts have been put into the design of real-time feedback controllers for voltage control purposes, see e.g. \cite{zhang2013local,bolognani2013distributed,li2014real,zhu2016fast,cavraro2016value,liu2018hybrid,tang2019fast,qu2019optimal,magnusson2020distributed}. %Such feedback controllers do not need real-time load/renewable generation or predictions; instead, they simply need voltage measurements and adjust the active/reactive power set point according to the voltage violation. For example, \cite{zhang2013local,li2014real} propose methods based on the integral controller; \cite{li2014real,bolognani2013distributed} propose feedback controllers based on the dual ascent method; \cite{qu2020optimal} proposes controllers based on the primal-dual method.  
Despite the progress, most of the existing work has only been able to optimize the steady state cost, i.e. the cost of the operating point after the voltage converges into the safe limit. In the meanwhile, transient performance is of equal importance. For example, once voltage violation happens, an important goal is to bring the voltage profile back to the safe limit as soon as possible, or in other words, to minimize the voltage recovery time. However,  optimizing or even analyzing the transient cost like the voltage recovery time has long been challenging as this is a nonlinear control problem. 
The challenge has further been complicated by the fact that many existing works \cite{li2014real,cavraro2016value,liu2018hybrid,tang2019fast,qu2019optimal,magnusson2020distributed} require knowledge of the topology and the parameters of the electric grid. Yet, such knowledge is not always available due to frequent system reconfigurations (resulting in topology change~\cite{weng2016distributed}) and time-varying system parameters resulting from facility aging, temperature and humidity change, etc. 

Reinforcement Learning (RL), having achieved impressive success in the past decade in game play~\cite{silver2016mastering}, robotics \cite{kalashnikov2018scalable}, is a promising tool to address the above challenges. RL methods do not need knowledge of explicit models and can learn from interactions with the underlying system. Further, due to the expressive power of neural networks as controllers/policies, RL is effective in learning nonlinear controllers with good transient performance. As a result, there has been tremendous interest in using RL for voltage control ~\cite{chen2020data,9353702,9328796,9143169,mukherjee2021scalable,kou2020safe,xu_optimal_2020,yang_two-timescale_2020,wang_data-driven_2020,wang_safe_2020,duan_deep-reinforcement-learning-based_2020,cao_multi-agent_2020,liu2020two}, see \cite{chen2021reinforcement} for a recent review. 

% Deep reinforcement learning (RL) has achieved impressive success in the past decade, highlighted by high-profile success stories such as in game play~\cite{silver2016mastering}. As a result, RL has been recognized as a promising alternative for more traditional decision and control tasks in real-world engineering systems, e.g. in robotics~\cite{kalashnikov2018scalable}, energy systems~\cite{chen2021reinforcement}, and transportation systems~\cite{wu2017flow}, among others.   
% However, despite the promise, major hurdles remain before deployment in such systems is feasible. Given the promising potential, a long line of work has studied 


Despite this interest, it has been generally agreed that the key challenge in applying RL to power systems is the \emph{stability} issue \cite{chen2021reinforcement}. 
Specifically, power systems are critical infrastructure systems that place a high emphasis on stability, i.e. the ability to maintain at safe operating points under disturbances. Stability is important because instability can lead to unsafe operating conditions that violate regulatory requirements \cite{regulator} or even lead to catastrophic consequences, e.g., blackouts \cite{haes2019survey}. 
%Further, with the proliferation of volatile renewable energy, the need for stability is becoming even more important.
%Consider power systems, for instance. Due to the proliferation of renewable energy and its intrinsic intermittency and stochasticity, current power systems face severe operational challenges~\cite{markard2018next}. %\cite{bird2013integrating,turitsyn2011options}. 
Despite the importance of stability, off-the-shelf RL algorithms lack provable stability guarantees. In particular, popular RL methods for continuous control, such as deep deterministic policy gradient (DDPG)~\cite{lillicrap2015continuous}, are gradient-based methods that focus on minimizing cost and do not explicitly consider stability. Even if the learned policy may appear ``stable'' on the training data set, it is not guaranteed to be stable as stability is a worst case concept requiring provably checking under the worst case scenario, which off-the-shell RL methods do not consider. 
The lack of provable stability guarantees is one of the biggest hurdles in applying RL to power systems since as mentioned earlier, instability can be catastrophic. 

%\guannan{I removed about the part on "in contrast, control theory can handle stability and we want to combine the two. "}

%\guannan{use power system as example } which are properties where off-the-shelf RL algorithms have well-known issues. In particular, popular RL methods for continuous control, like deep deterministic policy gradient (DDPG)~\cite{lillicrap2015continuous}, are gradient based methods that focuses on minimizing the cost and do not explicitly consider the stability. The lack of formal stability guarantees is an issue for safety critical systems since instability can cause catastrophic consequences, e.g., blackout in power systems. 

%In contrast, control-theoretic approaches provide a rich set of tools for analyzing the stability of dynamical systems and synthesizing control policies with formal stability guarantees. There is a large body of work that focuses on designing stable and robust controllers for linear systems and beyond \cite{zhou1996robust,dullerud2013course,lale2020explore}. For example, for general dynamical systems, Lyapunov's direct method provides a way to verify whether a system is stable or not, and can be utilized to synthesize stable controllers~\cite{khalil2002nonlinear}. Additionally, there are various other tools like contraction analysis \cite{lohmiller1998contraction} and passivity theory \cite{slotine1991applied} that guarantee stability. 

Motivated by the challenge above, the question we address in this paper is: \emph{Can we apply RL to voltage control with provable stability guarantee?} 

%This goal is similar in spirit to recent work that focuses on ensuring safety in RL via control theoretic methods such as barrier functions and Hamilton-Jacobi safety analysis, e.g., \adam{add cites}.  However, safety does not imply stability, and vice versa (though stability does imply asymptotic safety satisfaction).  Thus, ensuring stability requires fundamentally different tools than safety. 

%To this point, attempts to provide stability in RL have relied on Lyapunov-based policy learning, where the goal is to jointly learn the policy and the Lyapunov function, e.g., via a neural network~\cite{chang2019neural,jin2020neural}. However, learning a Lyapunov function is challenging, even when it is not coupled with policy learning. In this paper, we take a different approach and seek to build upon the principled approaches for constructing Lyapunov functions in the control theory literature to constrain policy learning in a way that, by design, guarantees stability conditions are met.

%\guannan{Need to be consistent on controller vs. policy}\yuanyuan{I changed some of them to policy?}

\textbf{Contributions.} We answer the question affirmatively by designing a stability constrained RL framework %\guannan{Can I say stable DDPG right at the beginning?} \yuanyuan{maybe say stability constrained reinforcement learning at the beginning - as our title is still for RL OR we want to change the title to stable DDPG?} 
that learns a control policy to optimize transient cost for voltage control with provable stability guarantees. The key idea underlying our approach is that we show strict monotonicity of the policy is sufficient to formally guarantee stability (Theorem~\ref{thm:voltage_stab}). The technique underlying Theorem~\ref{thm:voltage_stab} is that we derive an explicitly constructed Lyapunov function, which we use to certify stability for all monotone policies. With this stability result, we propose a Stable-DDPG approach which integrates the monotone constraint with DDPG through monotone policy network design (Corollary~\ref{corollary:stacked_relu}). 
The proposed method enables us to leverage the power of RL to improve the transient performance of voltage control without knowing the underlying model parameters, and in the meanwhile provably guarantee stability during and after the training. To the best of our knowledge, this is the first RL approach that learns nonlinear policies with stability guarantees for voltage control. %\guannan{Is is fair to say "this is the first RL approach that guarantee stability for voltage control" have a stronger ending sentence}

We also perform numerical case studies to demonstrate the effectiveness and stability of the proposed method with both simulated disturbances and real-world data. Our method guarantees voltage stability under all operating conditions, which is not true for the standard DDPG method. In addition, our method can reduce the transient control cost by more than 30\% and shorten the voltage recovery time by a third compared to a widely used linear policy in the literature \cite{li2014real,zhang2013local}. 
%policy learning with stable controller design in safety-critical systems, where Krasovskii's method is used to certify stability in settings such as communication network~\cite{feijer2009krasovskii,feijer2010stability}, transportation~\cite{peeta2003stability} and robotics~\cite{chung2009cooperative}. 
%\cite{feijer2009krasovskii,feijer2010stability}. \adam{Add a more concrete list with citations here where we cite various NUM problems, e.g.}
%where the Lyapunov function can be formed as the quadratic sum of the derivative of the state variables.
%\adam{Add a sentence of two about the generality of the models where the approach can be applied}
%\adam{Note broad applicability and then comment that we choose power...}

%We illustrate the use of the stability aware policy learning framework in a real-world safety-critical system: \emph{voltage control} in power systems.
%Voltage control is a challenging problem in power systems where traditional control approaches fail to achieve good performance at low control cost, and there has been a significant interest in using RL, e.g., \cite{chen2021reinforcement}. Yet a key issue that prevents RL from being deployed is stability. Voltage instability can violate regulatory requirements \cite{regulator} and even cause cascading failures \cite{haes2019survey}. We use our framework to design a policy with formal stability guarantees (Theorem~\ref{thm:voltage_stab}),

% \revise{Voltage control is a challenging problem in energy system where traditional control approaches fail to achieve good performance at low control cost, and there has been significant interests in using RL for voltage control. Yet a key issue that prevents RL been deployed is stability, as voltage instability can violate regulatory requirements and even causing cascading failures. In our paper, we use our framework to design a policy with formal stability guarantee, and perform various numerical case studies to demonstrate the effectiveness and stability of the proposed method with different simulated disturbances and real-world load and photovoltaic (PV) generation data. The proposed method guarantees the voltage stability under all operation conditions whereas standard RL fails to. In addition,
% our method can reduce the transient control cost by more than 34\% and shorten the voltage recovery time by a third, compared to widely used linear policy in the literature. }
%\adam{Fill in a few sentences about this problem since we want to get credit for a "real" application.}  In this case, we see \adam{say something about the improvement} \adam{really hit on voltage control being important and RL not being able to be applied without stability guarantee }

\textbf{Related Work.} This paper connects to a broad set of literature in RL, control, and power systems.

\textit{Lyapunov-based Policy Learning.} The Lyapunov theory is a systematic framework to analyze the stability of a control system. The core idea is to identify a positive definite function (i.e., a Lyapunov function) of the system’s state, with negative derivatives along system trajectories~\cite{khalil2002nonlinear}. 
Using Lyapunov functions in RL was first introduced by~\cite{perkins2002lyapunov}, but the work did not discuss how to find a candidate Lyapunov function in general except for a case-by-case construction. A set of recent works including~\cite{chang2019neural,jin2020neural,chow2018lyapunov,richards2018lyapunov,manek2020learning} have attempted to address this challenge by jointly learning the policy and the Lyapunov function, where \cite{chow2018lyapunov} uses linear programming and \cite{chang2019neural,jin2020neural,richards2018lyapunov,manek2020learning} parameterizes the Lyapunov function as neural networks. 
In the context of these works, our contribution can be viewed as explicitly constructing a Lyapunov function for the voltage control problem and using it to guide policy learning. 

%\textit{Safe Reinforcement Learning.} The goal of safe RL is to learn a policy that avoids entering unsafe regions, rather than requiring a policy to have attractive or bounded behavior. Various methods have been proposed to ensure safety in RL, see~\cite{garcia2015comprehensive} for a complete survey. In addition, many recent works focus on ensuring safety via control-theoretic methods such as using control barrier functions~\cite{taylor2020learning}, Hamilton-Jacobi safety analysis~\cite{fisac2019bridging}, and model predictive control as a safety filter~\cite{hewing2020learning}. We note that safety does not imply stability and vice visa. In some sense, stability is a more stringent requirement as it can lead to asymptotic safety satisfaction.

%\textit{Control Theory.} Our work is related to the Krasovskii's method \cite[Chapter 4]{khalil2002nonlinear} and contraction analysis \cite{lohmiller1998contraction}, which can be viewed as a specific way of constructing a Lyapunov function. More broadly, there are a large body of tools in control theory that synthesize controllers that are stable, e.g., passivity theory \cite{desoer1975feedback}, feedback linearization \cite{slotine1991applied}, model-predictive control \cite{rawlings2017model}, etc. In the context of these works, our contribution can be viewed as bridging one of these classical tools with policy learning in RL. 

\textit{Reinforcement Learning for Power Systems.} 
%Voltage control is a fundamental problem in the safe and efficient operation of power systems under high penetration of renewables. 
Our work contributes to a growing line of papers that use RL for voltage control~\cite{chen2020data,9353702,9328796,9143169,mukherjee2021scalable,kou2020safe,xu_optimal_2020,yang_two-timescale_2020,wang_data-driven_2020,wang_safe_2020,duan_deep-reinforcement-learning-based_2020,cao_multi-agent_2020,liu2020two}, see \cite{chen2021reinforcement} for a recent review. As pointed out in  \cite{chen2021reinforcement}, one of the key issues in RL for power system control is the lack of provable stability guarantees, and our work makes a step toward addressing this issue by providing a formal stability guarantee on the learned policy. In particular, our experiments compare against~\cite{wang_data-driven_2020}, which uses standard multi-agent DDPG for voltage control. Closest in spirit to our paper is~\cite{cui2020reinforcement}, which proposes a stable RL approach for frequency control via a Lyapunov approach. However, their approach only applies to the frequency control application, while our method works for voltage control which requires a different Lyapunov function design. Interestingly, both our work and prior work~\cite{cui2020reinforcement} arrive at a similar stability condition, that is strict policy monotonicity guarantees system stability. %\guannan{Any other difference from Baosen's work?}

%used \adam{We should probably say a bit more about the specific related work comparison in the case of voltage control...highlight baosen's work}
%for example \cite{xu_optimal_2020,wang_data-driven_2020,wang_safe_2020,duan_deep-reinforcement-learning-based_2020,cao_multi-agent_2020,liu2020two} [\todo{too much?}], 

==> Safe RL for Voltage Control (ACC)/Method.tex <==
We now introduce our main framework for stability constrained policy learning for voltage control. We start by stating our main result on the voltage control stability. We demonstrate the voltage stability constraint can be translated to a monotonicity constraint on the policy, which can be satisfied by smart design of monotone neural networks.

%\todo{High-level overview of the method}
%\todo{Explain how to enforce the stability via the monotonicity}
%However, in general RL algorithms like in DDPG, stability is not an explicit requirement. It is more like an implicit regularization, because instability usually leads to high (or infinite) costs. 
\subsection{Key Idea: Monotonicity Guarantees Stability}
As we mentioned in Section~\ref{sec:preliminary_ddpg}, the lack of an explicit stability requirement in standard RL algorithms can lead to several issues. During the training phase, the policy may become unstable, causing the training process to terminate. Even after a policy is trained, there is no formal guarantee that the closed loop system is stable, which hinders the learned policy's deployment in real-world power systems where there is a very strong emphasis on stability. In order to explicitly constrain stability in policy learning, we constrain the search space of policy in a subset of stabilizing controllers from Lyapunov stability theory. Interestingly, we show that monotone policy guarantees stability for voltage control, which is presented in Theorem \ref{thm:voltage_stab}.

%\yuanyuan{Describe about challenge: RL has no stability guarantee}
%\yuanyuan{Main contribution - monotone policy guarantees stability}
\begin{theorem}\label{thm:voltage_stab}
Suppose for all $i$, $g_{i,\theta_i}$ is a continuously differentiable function satisfying $g_{i,\theta_i}(v_i) = 0$ for $v_i \in [\underline{v}_i,\bar{v}_i]$. Further, suppose each $g_{i,\theta_i}$ is strictly monotonically decreasing on $(-\infty,\underline{v}_i]$ and $[\bar{v}_i,\infty)$, and satisfies $\lim_{v_i\rightarrow\infty} |g_{i,\theta_i}(v_i)| = \infty$. Then, the voltage stability defined in Definition~\ref{def:voltage_stability} holds.
\end{theorem}

Theorem \ref{thm:voltage_stab} shows that the voltage stability condition in~\eqref{eq_rl:constr} can be enforced by constraining the policy network to be monotone, which we will introduce in Section~\ref{sec:algorithm_design}.
The key technique that underpins Theorem \ref{thm:voltage_stab} is the Lyapunov stability theory, which involves defining a positive definite function $V(\cdot)$ that decreases along the system trajectory. 
Specially, we use Krasovskii's method~\cite{khalil2002nonlinear} for constructing the Lyapunov function. For the voltage control problem with dynamics $\dot{\mathbf{v}} = f(\mathbf{v}, \mathbf{u}) = X\mathbf{u}$ and $\mathbf{u} = g_\theta(\mathbf{v}) = [ g_{i,\theta_i}(v_i)]_{i\in\mathcal{N}}$, we consider the following Lyapunov function,
\begin{equation}\label{eq:Kra_func}
    V(\mathbf{v}) =\frac{1}{2} f(\mathbf{v}, g_{\theta}(\mathbf{v}))^\top X^{-1} f(\mathbf{v}, g_{\theta}(\mathbf{v}))
\end{equation}
where $X$ is a positive definite matrix by Proposition~\ref{prop:RX_pd}. A sufficient condition for the system to be stable is that, the derivative of the Lyapunov function~\eqref{eq:Kra_func} satisfies the following condition,
\begin{align}
    \frac{d}{dt} V(\mathbf{v}(t)) &=  (\nabla_{\mathbf{v}} {V}(\mathbf{v}))^\top \dot{\mathbf{v}} \nonumber \\
    &= \frac{1}{2} (X\mathbf{u})^\top  \Big[X^{-1} G(\mathbf{v},\theta) + G(\mathbf{v},\theta)^\top X^{-1} \Big] \nonumber\\
    & \quad \quad (X \mathbf{u}) < 0, \forall \mathbf{v} \notin \mathcal{S}_e  \label{eq:lyapunov_decreasing}
\end{align}
where $G(\mathbf{v},\theta) = \frac{\partial f(\mathbf{v}, \mathbf{u})}{\partial \mathbf{v}} + \frac{\partial f(\mathbf{v}, \mathbf{u})}{\partial \mathbf{u}} \frac{\partial \mathbf{u}}{\partial \mathbf{v}} = X\frac{\partial g_{\theta}(\mathbf{v})}{\partial \mathbf{v}}$ is the system Jacobian and $\mathcal{S}_e$ is the set of equilibrium points. This leads to our voltage stability condition, 
\begin{equation}
\label{eq:stability_LMI_Kra}
[\frac{\partial g_{\theta}(\mathbf{v})}{\partial \mathbf{v}} + \frac{\partial g_{\theta}(\mathbf{v})}{\partial \mathbf{v}}^\top \Big] \prec 0\,, \forall \mathbf{v} \notin \mathcal{S}_e 
\end{equation} 
In particular, since the controller is decentralized where $u_i(t) = g_{i,\theta_i}(v_i(t))$ only depends on local voltage measurement $v_i(t)$, the Jacobian matrix $\frac{\partial g(\mathbf{v})}{\partial \mathbf{v}}$ is diagonal with the $i$-th element as $\frac{\partial g_{i,\theta_i}(v_i)}{\partial v_i}$. Therefore, conditions~\eqref{eq:stability_LMI_Kra} can be met with each $g_{i,\theta_i}$ being strictly monotonically decreasing on $(-\infty,\underline{v}_i]$ and $[\bar{v}_i,\infty)$, and $g_{i,\theta_i}(v_i) = 0$ for $v_i \in [\underline{v}_i,\bar{v}_i]$. The detailed proof are as provided in Appendix~\ref{sec:proof}.

%For a dynamical system $\dot{x} = f(x, u)$ with $u = g_{\theta}(x)$, Krasovskii's method leads to the following Lyapunov function:
% \begin{equation}\label{eq:Kra_func}
%     V(x) =\frac{1}{2} f(x, g_\theta(x))^\top M f(x,g_\theta(x)).
% \end{equation}
% where $M$ is a positive definite matrix. A sufficient condition for the system to be stable is that, the derivative of the Lyapunov function~\eqref{eq:Kra_func} is negative definite along the system trajectory.
% \begin{align}
%     \frac{d}{dt} V(x(t)) &=  (\nabla_x {V}(x))^\top \dot{x} \nonumber \\
%     &=f(x, g_\theta(x))^\top M G(x, \theta) f(x, g_\theta(x)) \nonumber\\
%     &= \frac{1}{2} f(x, g_\theta(x))^\top  \Big[ M G(x,\theta) + G(x,\theta)^\top M \Big] \nonumber\\
%     & \quad \quad f(x, g_\theta(x)) < 0, \forall x \notin \mathcal{X}_e  \label{eq:lyapunov_decreasing}
% \end{align}
% where $G(x,\theta) = \frac{\partial f(x, u)}{\partial x} + \frac{\partial f(x, u)}{\partial u} \frac{\partial g_{\theta}(x)}{\partial x}$ is the system Jacobian and $\mathcal{X}_e$ is the set of equilibrium points. This leads to our general policy stability condition, 
% \begin{equation}
% \label{eq:stability_LMI_Kra}
% [M G(x,\theta) + G(x,\theta)^\top M \Big] \prec 0
% \end{equation} 
% In particular, for the proof of Theorem~\ref{thm:voltage_stab}, we choose $M = X^{-1}$ and conditions~\eqref{eq:stability_LMI_Kra} can be met with each $g_{i,\theta_i}$ is strictly monotonically decreasing on $(-\infty,\underline{v}_i]$ and $[\bar{v}_i,\infty)$, and $g_{i,\theta_i}(v_i) = 0$ for $v_i \in [\underline{v}_i,\bar{v}_i]$. Detailed proof are as provided in Appendix~\ref{sec:proof}.

\subsection{Algorithm Design}
\label{sec:algorithm_design}
The proposed stability-constrained policy learning algorithm works as follows. At every training iteration $k$, we randomly generate an initial states $\{v_i(0)\}$ for all nodes $i=1,...,N$. Then we use the current policy $g^{(k)}_{i, \theta_i}(v_i(t))$ to generate a trajectory of length $T$, and store the (state, action, reward, next state) data pairs in a replay buffer. Next, we use random samples from the replay buffer to update the policy and value networks following Eq.~\eqref{eq:policy_update} and Eq.~\eqref{eq:value_update}.
Specially, we parameterize the control policies $g_{i,\theta_i}(v_i), \forall i = 1,..., N$ via monotone neural networks with a deadband in $[\underline{v}_i,\bar{v}_i]$. As shown in Theorem \ref{thm:voltage_stab}, such design guarantees voltage stability.
%Theorem \ref{thm:voltage_stab} shows that the voltage stability condition in~\eqref{eq_rl:constr} can be enforced by restricting the policy to be monotone with respective to voltage $v_i$ except for a deadband in $[\underline{v}_i,\bar{v}_i]$. Thus, 

There are different approaches for monotone neural network architecture design in literature~\cite{sill1997monotonic,daniels2010monotone,cui2020reinforcement}.
In this paper we follow the monotonic neural network design in~\cite[Lemma 3]{cui2020reinforcement}, which used a single hidden layer neural network with $d$ hidden units and ReLU activation. 
\begin{corollary}(Stacked ReLU Monotone Network~\cite[Lemma 3]{cui2020reinforcement})
\label{corollary:stacked_relu}
 The stacked ReLU function constructed by Eq~\eqref{eq:relu_pos} is monotonic increasing for $x > 0$ and zero when $x \leq 0$.
\begin{subequations}\label{eq:relu_pos}
    \begin{align}
    \xi^{+}(x; w^+, b^+) &= {(w^+)^\top} \text{ReLU}(\mathbf{1} x + b^+)\\
    \text{where} & \sum_{i=1}^{l} w^{+}_i \geq 0, \forall l = 1, 2, ..., d\\
    & b^{+}_1 = 0, b^{+}_l \leq b^{+}_{l-1}, \forall l =2, 3, ..., d
    \end{align}
\end{subequations}
The stacked ReLU function constructed by Eq~\eqref{eq:relu_neg} is monotonic increasing for $x < 0$ and zero when $x \geq 0$.
\begin{subequations}\label{eq:relu_neg}
    \begin{align}
    \xi^{-}(x; w^{-}, b^{-}) &= (w^{-})^\top \text{ReLU}(-\mathbf{1} x + b^{-})\\
    \text{where} & \sum_{i=1}^{l} w^{-}_i \leq 0, \forall l = 1, 2, ..., d\\
    & b^{-}_1 = 0, b^{-}_l \leq b^{-}_{l-1}, \forall l =2, 3, ..., d
    \end{align}
\end{subequations}
\end{corollary}

Following Corollary~\ref{corollary:stacked_relu}, we parameterize the controller at bus $i$ as $g_{i,\theta_i}(v_i) = -[\xi_{\theta_i}^{+}(v_i) + \xi_{\theta_i}^{-}(v_i)]$ where $\xi_{\theta_i}^{+}(v_i): \mathbb{R} \rightarrow \mathbb{R}$ is monotonically increasing for $v_i >0$ and zero when $v_i \leq 0$, and $\xi_{\theta_i}^{-}(v_i): \mathbb{R} \rightarrow \mathbb{R}$ is monotonically increasing for $v_i <0$ and zero otherwise. In addition, to incorporate the dead-band within range $v_i \in [\underline{v}_i, \overline{v}_i]$, we can simply set $w^{+}_{1} = 0, b^{+}_{2} = -\overline{v}_i$ and $w^{-}_{1} = 0, b^{-}_{2} = -\underline{v}_i$. 
We demonstrate the effectiveness of this approach using a case study in the next section.
%For notational simplicity, we show the design for one policy and drop the dependence of $\xi^{+}, \xi^{-}$ on $i$. The following requirements on network weight $w \in \mathbb{R}^d$ and bias $b \in \mathbb{R}^d$ ensures monotonicity of $\xi^{+}(\cdot)$: 
% \begin{equation}\label{eq:relu_nn}
% \xi^{+}(x; w^+, b^+) = {(w^+)^\top} \text{ReLU}(\mathbf{1} x + b^+)
% \end{equation}
% where $\mathbf{1} \in \mathbb{R}^d$, $\sum_{i=1}^{l} w^{+}_i \geq 0, \forall l = 1, 2, ..., d$ and $b^{+}_1 = 0, b^{+}_l \leq b^{+}_{l-1}, \forall l =2, 3, ..., d$. Similarly,
% \begin{equation}\label{eq:relu_nn}
% \xi^{-}(x; w^{-}, b^{-}) = (w^{-})^\top \text{ReLU}(-\mathbf{1} x + b^{-})
% \end{equation}
% with $w^{-} \in \mathbb{R}^d$ and $b^{-} \in \mathbb{R}^d$ are the weight and bias vector of network $\xi^{-}$, with constraints $\sum_{i=1}^{l} w^{-}_i \leq 0, \forall l = 1, 2, ..., d$ and $b^{-}_1 = 0, b^{-}_l \leq b^{-}_{l-1}, \forall l =2, 3, ..., d$. 

%The final voltage controller is designed as the monotone network, with a dead-band within range $[\underline{v}_i, \overline{v}_i]$. %Once voltage converges within the lower and upper limits, the system is stable and no additional control is needed. 
%The dead-band can be easily satisfied by setting $w^{+}_1 = 0, b^{+}_2 = -\overline{v}_i$ and $w^{-}_1 = 0, b^{-}_2 = -\underline{v}_i$. 
%We demonstrate the effectiveness of this approach using a case study in the next section.

% In contrast to the classical applications of Krasovskii's method to certify stability for autonomous systems, in which case the system Jacobian itself satisfies the negative definiteness requirement, our framework combines  \eqref{eq:stability_LMI_Kra} with policy optimization to learn policies that can stabilize complex and uncertain dynamical systems that are not stable without control. The main benefit of our approach is to constrain policy learning via a well-defined stability condition. Existing works seek to jointly learning the Lyapunov function and policy~\cite{chang2019neural,jin2020neural}.  In contrast, Krasovskii's method provides a candidate for the Lyapunov function of dynamical systems of the form~\eqref{eq:sysdyn}, namely $V = f^\top Mf$. This leads to a concrete stability constraint on the Jacobian of the policy, which we show can be enforced in some classes of system via monotone policy network design in the discussion that follows. The approach also integrates smoothing into policy learning because it guarantees stability both during training and testing, with natural generalizability to all trajectories as other types of Lyapunov-based methods. 

% \textbf{Discussion.} In this paper we focus on using Krasovskii's method to generate a Lyapunov function for voltage control, and constrain the policy learning for stability guarantee. We note that although we focus on the voltage control problem, the proposed framework can also be applied in broader systems with proper adaption. In particular, Krasovskii's method is related to contraction analysis \cite{lohmiller1998contraction} where the matrix $M$ is allowed to depend on $t$, and the corresponding stability condition is  
% \[ \forall t, M(t) G(x,\theta) + G(x,\theta)^\top M(t) + \frac{d}{dt}M(t)\preceq -\nu M(t), \]
% for some $\nu>0$. This can be viewed as a generalization of the Krasovskii's method and has been widely used in robotic manipulation and locomotion tasks~\cite{chung2009cooperative}.


%Studying how to incorporate this more general condition into RL is an interesting future direction. Another approach for broadening the applicability of the approach is jointly learn system dynamics with uncertainty quantification and the primal-dual approach to provide a formal stability guarantee.  
%Another approach for broadening the applicability of the approach is for systems that don't have the properties as Corollary~\ref{cor:monotone} and the system dynamics are unknown. It jointly learn system dynamics with uncertainty quantification and the primal-dual approach to provide a formal stability guarantee.


% \guannan{1. explicit construction of Lyapunov, novelty is directly learning Lyapunov is hard, this explit construction easier to implement in learning? 2. Krasovskii's method is originally for autonomous systems,  3. }

% \adam{This proof still needs work... we should add more context/intuition to it and write it in a way that highlights what is "new" and what is just the standard version of the approach. I.e., what is the novelty that allows it to be integrated with learning}

% \yuanyuan{Also discuss limitations of our method: Kravskii's method can also be used in some systems}

% \emph{Proof of Theorem~\ref{thm:stability_Kra}}. The main idea is to use the Krasovskii's method~\cite[Chapter 4]{khalil2002nonlinear} to construct a Lyapunov function that certifies stability. 
% %Let $\dot{x} = f(x,u)$ be a dynamical system, with $x$ being the state and $u$ being the input. 
% Specifically, given the controller $u = g_\theta(x)$, we consider the following Lyapunov function:
% \begin{equation}
%     V(x) =\frac{1}{2} f(x,g_\theta(x))^\top M f(x,g_\theta(x)),
% \end{equation}
% where $M$ is the positive definite matrix in the constraint \eqref{eq:stability_LMI_Kra}. Then, we can calculate,
% \[\nabla_x {V}(x) =[\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x} ]^\top M f(x,g_\theta(x)), \]
% and further,
% \begin{align}
%     \frac{d}{dt} V(x(t)) &=  f(x,g_\theta(x))^\top M [\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x} ] \dot{x} \nonumber \\
%     &=f(x,g_\theta(x))^\top M [\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x} ] f(x,g_\theta(x)) \nonumber\\
%     &= \frac{1}{2} f(x,g_\theta(x))^\top  \Big[ M[\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x}] \nonumber\\
%     &\qquad + [\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x}]^\top M \Big] f(x,g_\theta(x)) \leq 0,  \label{eq:lyapunov_decreasing}
% \end{align}
% where we have used condition~\eqref{eq:stability_LMI_Kra}. Also, note that $V(x)\geq 0$, and $V(x) = 0$ if and only of $x\in S_e$. Lastly, if a trajectory $x(t)$ is such that $\frac{d}{dt} V(x(t)) = 0, \forall t\geq 0$, then we must have $f(x(t),g_\theta (x(t))) = 0$ for all $t$, i.e. $x(t)\in S_e$ for all $t$. Therefore, by LaSalle's Invariance Principle, we must have $S_e$ is asymptotically stable. 

% If $\Vert f(x,g_\theta(x))\Vert\rightarrow\infty$ as $\Vert x\Vert\rightarrow \infty$, we have $V(x)\rightarrow\infty$ as $\Vert x\Vert\rightarrow\infty$, i.e. $V$ is radially unbounded. Then again by LaSalle's Invariance Principle, the system is globally asymptotically stable around $S_e$, which finishes the proof of Theorem~\ref{thm:stability_Kra}. \qed



%Therefore, if the symmetrized matrix of $M[\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x}]$ is negative definite, i.e.
% \begin{align*}
%     M[\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x}] + [\frac{\partial f(x,g_\theta(x))}{\partial x} + \frac{\partial f(x,g_\theta(x))}{\partial u} \frac{\partial g_\theta(x)}{\partial x}]^\top M \prec 0,
% \end{align*}
%then by LaSalle invariance principle, the set of accumulation points of the trajectories must be contained in the set $\{x: f(x,g_\theta(x)) = 0\}$. If the set $\{x: f(x,g_\theta(x)) = 0\}$ is the set of the desired equilibrium points, then $\eqref{eq:stability_LMI_Kra}$ is a sufficient condition for stability. %We provide a complete proof of Theorem~\ref{thm:stability_Kra} in Appendix.
%The results above has been proven in various textbooks, and is summarized below. For completeness, we also provide a proof in the appendix X. 
% \begin{proposition}
% When \eqref{eq:stability_LMI_Kra} holds, we have the accumulation points of the trajectory for dynamical system $\dot{x} = f(x,g(x))$ must be contained in the set $\{x:f(x,g(x)) = 0\}$. 
% \end{proposition}

% The above stability condition \eqref{eq:stability_LMI_Kra} provides a natural way to guarantee stability in policy learning in RL. Specifically, 
% if we can place constraints on the policy class such that \eqref{eq:stability_LMI_Kra} always holds, then we have a stability guarantee. However, the condition \eqref{eq:stability_LMI_Kra} involves $ \frac{\partial f(x,u)}{\partial x}$ and $ \frac{\partial f(x,u)}{\partial u}$, which is not known if $f$ is unknown. In what follows, we show that in many applications, there will be prior knowledge regarding $f$ which results in the condition~\eqref{eq:stability_LMI_Kra} being easily embedded in controller design. 

%\todo{Discuss more about this connection?}

==> Safe RL for Voltage Control (ACC)/Preliminary.tex <==


% as summarized in the following proposition, though it leaves open the task of constructing such a Lyapunov function.
% \begin{proposition}[Lyapunov functions for stability~\cite{khalil2002nonlinear}]
% Consider a control system in~\eqref{eq:dyn} with equilibrium point $x_e$, i.e., $f(x_e, g_\theta(x_e)) = 0$. Suppose there exists a continuously differentiable function $V: \mathbb{R}^n \rightarrow \mathbb{R}$ such that
% \begin{align}
%     V(x_e) &= 0 \text{ and } V(x) > 0,\forall x\in \mathcal{D}-\{x_e\}\\
%     \dot{V}(x) &< 0,\forall x\in \mathcal{D}-\{x_e\}
% \end{align}
% Then the system is asymptotically stable at the equilibrium point $x_e$ and $V$ is called a Lyapunov function. If $V$ is further radially unbounded, i.e. $V(x)\rightarrow\infty$ as $\Vert x\Vert\rightarrow\infty$, then the system is globally asymptotically stable around $x_e$. 
%\end{proposition}

%This calls to the question on how to formally ensure stability during policy learning, and how to guarantee the learned policy is guaranteed to be stable. This will be the focus of the next section. 

==> Safe RL for Voltage Control (ACC)/Voltage.tex <==
In this section, we first introduce the distribution system power flow models and the voltage control problem formulation. Then, we review some background for policy optimization in reinforcement learning.
\vspace{-12pt}
\subsection{Branch Flow Model for Distribution Networks}
\label{sec:voltage_control_formuation}
%We consider a standard voltage control formulation in power distribution networks. 
%We start with the system model: 
We consider the distribution network as a tree-structured graph $\mathcal{G} = (\mathcal{N},\mathcal{E})$, which consists of a set of nodes $\mathcal{N}_0=\{0,1,\ldots,n\}$ and edges $\mathcal{E}$, where node $0$ is the substation. We use $\mathcal{N} = \mathcal{N}_0/\{0\}$ to denote the set of nodes excluding the substation node. See Fig. \ref{fig1:vol_ctrl} for an example 5-bus network.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.25\textwidth]{pf_diagram.png}
    \caption{A 5-bus radial distribution network.}
    \label{fig1:vol_ctrl}
\end{figure}
%The tree is rooted at node $0$, the so-called substation.
%where there is a power distribution network, consisting of a set of $\mathcal{N}_0 = \{0,1,\ldots,n\}$ nodes, and an underlying graph $\mathcal{G} = (\mathcal{N}_0,\mathcal{E})$, which is a tree rooted at node $0$. 
Each node $i\in\mathcal{N}$ is associated with an active power injection $p_i$, a reactive power injection $q_i$, and a voltage magnitude $v_i$. We use $p, q$ and $v$ to denote the $p_i,q_i,v_i$ stacked into a vector. We consider the linear distribution power flow model, known as the Simplified Distflow model, which is a linear approximation of the underlying nonlinear branch flow model in radial distribution networks~\cite{baran1989network} by neglecting the quadratic power loss terms. The Simplified Distflow model is a commonly used model in the voltage control literature, see e.g.~\cite{li2014real,cavraro2016value,liu2018hybrid,tang2019fast,qu2019optimal,magnusson2020distributed} and the references therein. In the Simplified Distflow model, $p$, $q$ and $v$ satisfy the following equations, $\forall j \in\mathcal{N}, i=\textrm{parent}(j)$, \begin{subequations}
{\small
\begin{align}
    -p_j &= P_{ij}  - \sum_{k: (j, k) \in \mathcal{E}} P_{jk}\,, \quad
    -q_j = Q_{ij} - \sum_{k: (j, k) \in \mathcal{E}} Q_{jk}\,, \label{eq:conserv_law}\\
    -v_j &= v_i - 2(r_{ij}P_{ij} + x_{ij} Q_{ij})\,, (i, j) \in \mathcal{E} \label{eq:bfm_v}
\end{align}}
\end{subequations}
% \end{minipage}
%We consider the linear distribution power flow model~\cite{li2014real}, which is a widely adopted model for system analysis. 
%Consider a distribution grid, consisting of a set of $\mathcal{N}_0 = \{0,1,\ldots,n\}$ nodes, and a underlying graph $\mathcal{G} = (\mathcal{N}_0,\mathcal{E})$, which is a tree rooted at node $0$. In the graph, node $0$ is known as the substation, and all the other node are buses that correspond to residential areas. We also use $\mathcal{N} = \mathcal{N}_0/\{0\}$ to denote the set of nodes excluding the substation node. 
%Each node $i\in\mathcal{N}$ is associated with an active power injection $p_i$, and a reactive power injection $q_i$, as well as voltage magnitude $v_i$. We also use notation $p, q$ and $v$ to denote the $p_i,q_i,v_i$ stacked into a vector. We consider the linear distribution power flow model, which is a widely adopted model for power flow analysis. $p$ and $q$ and the voltage $v$ satisfies the following equations, $\forall j \in\mathcal{N}, i=\textrm{parent}(j)$, 
% \begin{subequations}
% \begin{align}
%     -p_j &= P_{ij} - r_{ij} {l_{ij}} - \sum_{k: (j, k) \in E} P_{ij}, \label{eq:bfm_p}\\
%     -q_j &= Q_{ij} - x_{ij} {l_{ij}} - \sum_{k: (j, k) \in E} Q_{ij}, \label{eq:bfm_q}\\
%     v_j &= v_i - 2(r_{ij}P_{ij} + x_{ij} Q_{ij}) + (r_{ij}^2 + x_{ij}^2) l_{ij}, \label{eq:bfm_v} \\
%     l_{ij} &= \frac{P_{ij}^2 + Q_{ij}^2}{v_i}, \label{eq:bfm_l}
% \end{align}
% \end{subequations}
%where $l_{ij}$, $P_{ij}$ and $Q_{ij}$ are additional variables representing the current, active power, reactive power flow on line $(i,j)$ respectively. Briefly speaking, equation  \eqref{eq:bfm_p} and \eqref{eq:bfm_q} present the power conservation at node $j$, and \eqref{eq:bfm_v} represent the voltage drop from node $i$ to node $j$, and lastly \eqref{eq:bfm_l} relates the current $l_{ij}$ magnitude to the power flows. 
% For theoretic derivation purposes, we will use the following linear approximation of the branch flow model. For most distribution grids: $r_{ij}, x_{ij} \ll 1$ and $v_j \approx 1$, we can neglect the higher order power loss term by setting $l_{ij} = 0$ and obtain the following linear approximation.
% \begin{subequations}
% \begin{align}
%     -p_j &= P_{ij}  - \sum_{k: (j, k) \in E} P_{ij},\quad \forall j \in\mathcal{N}, i=\textrm{parent}(j) \label{eq:bfm_p}\\
%     -q_j &= Q_{ij} - \sum_{k: (j, k) \in E} Q_{ij}\,, j = 1, ..., n \label{eq:bfm_q}\\
%     -v_j &= v_i - 2(r_{ij}P_{ij} + x_{ij} Q_{ij}) \label{eq:bfm_v}
% \end{align}
% \end{subequations}
In Equation~\eqref{eq:conserv_law}, $P_{ij}$ and $Q_{ij}$ represent the active power and reactive power flow on line $(i,j)$, and $r_{ij}$ and $x_{ij}$ are the line resistance and reactance. Briefly speaking, Equation~\eqref{eq:conserv_law} presents the power conservation law at node $j$, e.g., in Figure~\ref{fig1:vol_ctrl}, the power inflow at node 2 (orange) equals to the power outflow at node 2 (blue). Equation \eqref{eq:bfm_v} models the voltage drop from node $i$ to node $j$. 
The above equation can also be rearranged and written in the vector form~\cite{li2014real}:
\begin{equation}
\mathbf{v} = R \mathbf{p} + X \mathbf{q} + \mathbf{v}_0 \mathbf{1} = X\mathbf{q} + \mathbf{v}^{env}. \label{eq:lindistflow}
\end{equation}
Here we separate the voltage magnitude $\mathbf{v}$ into two parts: the controllable part $X\mathbf{q}$ that can be adjusted via adjusting reactive power injection $\mathbf{q}$ through various control devices, and the non-controllable part $\mathbf{v}^{env} = R\mathbf{p}+\mathbf{v}_0$ that is decided by the load and PV power $\mathbf{p}$. Matrix $R, X$ are given as follows, $R_{ij} = 2 \sum_{(h, k) \in P_i \cap P_j} r_{hk}\,, X_{ij} = 2 \sum_{(h, k) \in P_i \cap P_j} x_{hk}$, where $P_i$ is the set of lines on the unique path from the substation to bus $i$. Matrix $X$ and $R$ satisfy the following property, which is crucial for the stable control design. %in our ability to embed the stability condition \eqref{eq:stability_LMI_Kra} in controller design. .


%where $\mathbf{1}$ is the all one vector in $\mathbb{R}^n$, $v^{env} = Rp+v_0$. 

\begin{proposition}\label{prop:RX_pd}
Suppose $x_{ij}, r_{ij}>0$ for all $(i,j)$. Then, $X$ and $R$ are positive definite matrices. 
\end{proposition}

\subsection{Voltage Control Problem Formulation}
The goal of voltage control is to design control to lead the system voltage to reach the acceptable range $[\underline{v}, \overline{v}]$ under any system operating conditions at the lowest cost. Formally, voltage stability is defined as follows.
\begin{definition}[Voltage stability]
\label{def:voltage_stability}
The closed loop system is stable if for any $\mathbf{v}^{env}$ and $\mathbf{v}(0)$, we have $\mathbf{v}(t)$ converges to the set $S_{v} = \{ \mathbf{v}\in\mathbb{R}^n: \underline{v}_i\leq v_i \leq\bar{v}_i \}$ in the sense that $\lim_{t\rightarrow\infty }\dist(\mathbf{v}(t),S_v) = 0$ and the distance is defined as $\dist(\mathbf{v}(t),S_v) = \min_{\mathbf{v}' \in S_v}||\mathbf{v}(t)-\mathbf{v}'||$.
\end{definition}
% \textbf{Voltage Stability. }Voltage stability is defined as the ability of the system voltage trajectory to return to an acceptable range after a disturbance, cf. Definition~\ref{def:voltage_stability} below. Here the acceptable voltage range at node $i$ is an interval $[\underline{v}_i,\bar{v}_i]$, and $\underline{v}_i,\bar{v}_i$ are the voltage lower and upper limits, respectively, which are specified by regulatory requirements \cite{regulator}.
Violations of the acceptable voltage range are often caused by a sudden change in the load or the generation, which can damage the appliances of the end users and even cause cascading failures if the system cannot return to the range promptly \cite{haes2019survey}. Therefore voltage stability is a vital requirement for the safe operation of the power systems. 

With the requirement for voltage stability, the optimal voltage control problem can be formulated as follows,
%\guannan{I suggest we can make the cost to be general and this cost below is just an example. One can replace it with other costs.} \yuanyuan{Good point! Revised}
% \textbf{Voltage Control Problem.} The voltage control problem can be formulated as follows. 
% \begin{subequations}\label{opt:voltage_ctrl}
% \begin{align}
% \min & \int_{t=0}^{\infty} \gamma^t \sum_{i=1}^n c({v}_i(t), q_i(t)) dt \label{eq_rl:obj}\\
% \text{s.t.}\quad & v(t) = Xq(t) + v^{env} \label{eq_rl:dyn}\\
% & \dot{q}_i(t) = u_i(t) \label{eq_rl:policy}\\
% & \text{Voltage stability holds.}\label{eq_rl:constr}
% \end{align}
% \end{subequations}
\begin{subequations}
\label{opt:voltage_ctrl}
\begin{align}
\min_{\mathbf{\theta}} \quad & J(\theta)= \int_{t=0}^{\infty} \gamma^t \sum_{i=1}^n c_i({v}_i(t), u_i(t)) dt \label{eq_rl:obj}\\
\text{s.t.}\quad & \mathbf{v}(t) = X\mathbf{q}(t) + \mathbf{v}^{env} \label{eq_rl:dyn}\\
& \dot{q}_i(t) = u_i(t) = g_{\theta_i}(v_i(t))\label{eq_rl:policy}\\
& \text{Voltage stability holds.}\label{eq_rl:constr}
\end{align}
\end{subequations}
The goal of the voltage control problem is to reduce the total cost \eqref{eq_rl:obj}, which consists of two parts: the cost on voltage deviation and the cost of control actions. In particular, we consider $c_i({v}_i(t), u_i(t)) = \eta_1 [\max(v_i(t) - \bar{v}_i,0) + \min(v_i(t) - \underline{v}_i,0)]^2 + \eta_2 (u_i(t))^2$. Here $\eta_1, \eta_2$ are coefficients that balance the cost of action with respect to the voltage deviation.
We can set different $\eta_1, \eta_2$ at different nodes, and for simplicity, we choose the same $\eta_1,\eta_2$ across all nodes in the paper. 
%$\eta$ is a coefficient that balances the cost of action with respect to the voltage deviation. Note that we can set different $\eta$ at different nodes, and for simplicity, we choose the same $\eta$ across all nodes in the paper. 
Voltage dynamics of power system are represented by the power flow equation~\eqref{eq_rl:dyn}.  We envision that the reactive power control loop is embedded in an inverter control loop and operate at very fast timescales. Therefore, we use a continuous-time system to model the voltage/reactive power dynamics (unlike the more conventional discrete-time model). The control action $u_i$ means the rate of change of the reactive power injection $q_i$ in equation~\eqref{eq_rl:policy}, and we focus on the class of decentralized polices, $u_i(t) = g_{i,\theta_i}(v_i(t))$ only depends on local voltage measurement $v_i(t)$. Here $\theta_i$ is the policy parameter for the local policy $g_{i,\theta_i}$, and $\theta = (\theta_i)_{i\in\mathcal{N}}$ is the collection of the local policy parameters and is also the decision variable in \eqref{opt:voltage_ctrl}.

%\todo{Remark. (Guannan: comment on related work and difference)
%}

\textit{Transient cost vs. stationary cost. } Our problem formulation is different from those in the literature \cite{zhang2013local,bolognani2013distributed,li2014real,zhu2016fast,cavraro2016value,liu2018hybrid,tang2019fast,qu2019optimal,magnusson2020distributed} in the sense that the existing works typically consider the cost in stationarity, meaning the cost is evaluated at the fixed point or stationary point of the system. In contrast, our work considers the transient cost evaluated along the system trajectory, which is also an important metric for the performance of voltage control.
An important future direction is to unify these two perspectives and design policies that can optimize both transient and stationary costs. 

%\textit{Continuous time vs discrete time. } Another difference between is that we adopt a continuous time dynamics for the controller ($\dot{q}_i (t)= u_i(t)$), where in the literature, typically a discrete time dynamics is used. The continuous time dynamics can be applied because... 

\subsection{Existing Work: DDPG for Optimal Voltage Control}
\label{sec:preliminary_ddpg}
In order to solve the optimal voltage control problem in \eqref{opt:voltage_ctrl}, one need the exact system dynamics, i.e., $X$. However, for distribution system, the exact network parameters are often unknown or hard to estimate in real systems~\cite{chen2020data}. Further, \eqref{opt:voltage_ctrl} is a nonlinear control problem 
%is an infinite dimensional problem. In addition, when the exact system model and cost functions are not known to the local controllers, it is hard to use conventional optimization techniques to obtain the optimal controller. 
Reinforcement learning provides a powerful paradigm for solving \eqref{opt:voltage_ctrl}, by training a policy that maps the state to action via interacting with the environment, so as to minimize the loss function defined as~\eqref{eq_rl:obj}. 
%In particular, we parameterize each of the controller, i.e., $u_i(t) = g_{i,\theta_i}(v_i(t))$ as a neural network with weights $\theta_i$, which maps the local voltage $v_i(t)$ to local reactive power change $u_i(t)$.

There are many RL algorithms to solve the policy minimization problem \eqref{opt:voltage_ctrl}. In this paper, we focus on the class of RL algorithms called policy optimization. Generally speaking, the procedure is to run gradient methods on the policy parameter $\theta$ with step size $\eta$,
$ \theta \leftarrow \theta - \eta \nabla J(\theta). $
To approximate the gradient $\nabla J(\theta)$, one can use sampled trajectories such as REINFORCE~\cite{williams1992simple} or value function approximation such as actor-critic methods \cite{konda2000actor}. As we are dealing with deterministic policies, one of the most popular choices is the Deep Deterministic Policy Gradient (DDPG)~\cite{lillicrap2015continuous}, where the policy gradient is approximated by
\begin{equation}
\label{eq:policy_update}
\nabla J(\theta) \approx \frac{1}{N} \sum_{i\in B} \nabla_u \hat{Q}_{\phi}(v, u)|_{v = v[i], u=g_{\theta}(v[i])} \nabla_{\theta} g_{\theta}(v)|_{v[i]}\,,
\end{equation}
where $g_{\theta}(v)$ is the actor network, and $\{v[i], u[i]\}_{i\in B}$ are a batch of samples with batch size $|B| = N$ sampled from the replay buffer which stores historical state-action transition tuples. 
Here $\hat{Q}_{\phi}(v, u)$ is the value network (a.k.a critic network) that can be learned via temporal difference learning,
\begin{equation}
    \label{eq:value_update}
    \min_{\phi} L(\phi) = E_{(v, u, r, v')} [Q_{\phi}(v, u) - (r+\gamma Q_{\phi}(v', g_{\theta}(v'))]
\end{equation}
where $v'$ is system voltage after taking action $u$ and realization of $v^{env}$.
For more details of DDPG, readers could refer to~\cite{lillicrap2015continuous}. There have been a growing line of papers that use RL for voltage control~\cite{chen2020data,wang_data-driven_2020,wang_safe_2020}. In particular, ~\cite{wang_data-driven_2020} uses standard multi-agent DDPG for voltage control. However, in standard DDPG, stability is not an explicit requirement. It is more like an implicit regularization, because instability usually leads to high (or infinite) costs. Next, we will introduce our framework that guarantees stability in policy learning.

 
